Peculiar prompt emission and afterglow in H.E.S.S. detected GRB 190829A

We present the results of a detailed investigation of the prompt and afterglow emission in the HESS detected GRB 190829A. Swift and Fermi observations of the prompt phase of this GRB reveal two isolated sub-bursts or episodes, separated by a quiescent phase. The energetic and the spectral properties of the first episode are in stark contrast to the second. The first episode, which has a higher spectral peak of $\sim 120\:\text{keV}$ and a low isotropic energy $\sim 10^{50}\:\text{erg}$ is an outlier to the Amati correlation and marginally satisfies the Yonetoku correlation. However, the energetically dominant second episode has lower peak energy and is consistent with the above correlations. We compared this GRB to other low luminosity GRBs (LLGRBs). Prompt emission of LLGRBs also indicates a relativistic shock breakout origin of the radiation. For GRB 190829A, some of the properties of a shock breakout origin are satisfied. However, the absence of an accompanying thermal component and energy above the shock breakout critical limit precludes a shock breakout origin. In the afterglow, an unusual long-lasting late time flare of duration $\sim 10^4\:\text{s}$ is observed. We also analyzed the late-time \fermi-LAT emission that encapsulates the H.E.S.S. detection. Some of the LAT photons are likely to be associated with the source. All the above observational facts suggest GRB 190829A is a peculiar low luminosity GRB that is not powered by a shock breakout, and with an unusual rebrightening due to a patchy emission or a refreshed shock during the afterglow. Furthermore, our results show that TeV energy photons seem common in both high luminosity GRBs and LLGRBs.

==> GRB 190829A arxiv22May/table_SED.tex <==
\begin{table*}
\begin{center}
\renewcommand{\arraystretch}{1}\addtolength{\tabcolsep}{3pt}
\caption{The best-fit values of spectral and temporal indices for episodes marked in Figure \ref{fig:multiwavelength_lc}.}
\begin{tabular}{ |c | c  c c c | c c c c|}
 \hline 
\tiny{X-rays} &  \tiny{Intervals ($\rm s$) from}  & \tiny{Index}    & \tiny{ -$\rm log(L)/(n, k)$} & \tiny{Index}  & \tiny{Intervals ($\rm s$) from} & \tiny{Index} &\tiny{ -$\rm log(L)/(n, k)$} & \tiny{Index}\\ &
\tiny{Flux ($\rm erg ~cm^2 ~s^{-1}$)} & \tiny{$\rm \alpha$}  &  & \tiny{$\rm \beta$} & \tiny{Flux $\rm @$ 10 $\rm keV$ ($\rm Jy$ $@ 10 ~ \rm keV$)} & \tiny{($\rm \alpha_X$)}   &\tiny{}  & \tiny{($\rm \beta_X$)} \\ 
\hline
\tiny{I}   	        & \tiny{89.54 - 147.93}  & \tiny{$2.99_{-0.30}^{+0.20}$}  	&  \tiny{362/(16, 3)} &\tiny{$1.18_{-0.24}^{+0.26}$} & --- &--- & --- & ---\\	

\tiny{II}   	        & \tiny{147.93 - 619.84}  & \tiny{---} 	&  \tiny{---} & \tiny{$1.46_{-0.22}^{+0.23}$} & --- & --- & --- & ---\\	

\tiny{III}    	        &  \tiny{619.84 - $2.37 \times 10^{4}$}  & \tiny{$-2.82_{-0.20}^{+0.18}$}		& \tiny{---}  & \tiny{$1.02_{-0.06}^{+0.06}$} & \tiny{620 - 1140 } & \tiny{$-3.30_{-0.05}^{+0.12}$}& \tiny{584/(49, 3)} &\tiny{$1.18_{-0.21}^{+0.22}$}  \\	
\tiny{} & \tiny{$\rm t_b$ = $1570_{-67}^{+68}$}   	& \tiny{$1.43_{-0.05}^{+0.05}$} & \tiny{16425/(449, 5)}  	&\tiny{$1.05_{-0.09}^{+0.09}$} &  \tiny{4860 - $2.37 \times 10^{4}$}		& \tiny{$1.80_{-0.06}^{+0.05}$} &\tiny{1988/(155, 3)} &\tiny{$1.01_{-0.09}^{+0.09}$}   \\	%\cdashline{}    

\tiny{IV}    	        & \tiny{$2.37 \times 10^{4}$ - $9.60 \times 10^{5}$}  & \tiny{$1.02_{-0.03}^{+0.03}$}& \tiny{---}	 &\tiny{$1.13_{-0.09}^{+0.09}$}	 & \tiny{$2.37 \times 10^{4}$ - $1.55 \times 10^{6}$} & \tiny{$0.90_{-0.10}^{+0.10}$} & ---& \tiny{$1.02_{-0.11}^{+0.12}$}   \\	
& \tiny{$\rm t_b$ = $3.95_{-1.28}^{+2.39}$ $\times10^{5}$}  & \tiny{$1.33_{-0.29}^{+0.13}$}	& \tiny{5053/(190, 5)} &\tiny{$1.32_{-0.24}^{+0.25}$}  & \tiny{$\rm t_b$ = $1.67_{-0.3}^{+0.4} \times 10^{5}$} & \tiny{$1.97_{-0.11}^{+0.12}$}  & \tiny{3301/(200, 5)}   & \tiny{$1.35_{-0.13}^{+0.13}$}\\ 
\tiny{IV $\rm-V^b$}   & \tiny{$9.60 \times 10^{5}$ - $7.90 \times 10^{6}$} & \tiny{$1.1_{-0.1}^{+0.1}$}  & \tiny{4031/(154, 3)} & \tiny{$1.05_{-0.26}^{+0.28}$ }& \tiny{$2.37 \times 10^{4}$ - $6.87 \times 10^{6}$} & \tiny{$1.22_{-0.03}^{+0.03}$} & \tiny{2468/(155, 3)} & \tiny{$1.21_{-0.1}^{+0.1}$}
\\
\hline
\end{tabular}
\label{tab:table_SED1}
\end{center}
%\setlength{\tabcolsep}{2pt}

We use power law %\footnote{\begin{equation*}
 %Flux \propto t^{\rm -\alpha}
%\end{equation*}}
or a smooth broken power-law (SBPL) \footnote{\begin{equation*}
Flux \propto \left[\left(\frac{t}{t_{\rm
b}}\right)^{\rm \alpha_1s} +\left(\frac{t}{t_{\rm
b}}\right)^{\rm \alpha_2s}\right]^{\rm -1/s} 
\end{equation*}
$\rm s$: smoothness parameter, $\rm \alpha_1$: index before break $\rm t_b$ and $\rm \alpha_2$: index after break  \citep{wang18:jet}, $\rm log(L)$: log-likelihood, n: number of data points and k: number of the free parameters in the fit. \\ $\rm b$: excluding $3 \times 10^5$ s - $2 \times 10^{6}$ s.
} function to model the XRT light curves for different segments using {\it python} module \sw{emcee}\citep{emcee}. All quoted errors on spectral parameters correspond to 16th and 84th percentiles.



\end{table*}
%
%








%\begin{table}
%\centering \renewcommand{\arraystretch}{2}\addtolength{\tabcolsep}{3pt}
%\caption{The best-fit values of the temporal PL indexes and spectral indices derived from the XRT Flux\@10 $keV$  light curve and spectrum of GRB 190829A.}
%\label{table2}
%\begin{tabular}{c  c  c c c c}
% \hline \hline
%\tiny{X-rays} &\hspace{0.5cm}   \tiny{Interval}  &\hspace{0.5cm}   \tiny{Index}  &  & \hspace{0.5cm} \tiny{ $log(L)/(n, k)$} & \hspace{0.5cm} \tiny{Temporal Model}\\ 
%\tiny{} & \hspace{0.5cm} \tiny{(s)} & \hspace{0.5cm}  \tiny{($\alpha_{\rm X}$)}   &  \tiny{($\beta_{\rm X}$)} & &\hspace{0.5cm}\tiny{($t_{b}$)} & \\ 
%\hline \hline
%\tiny{I}   	        & \hspace{0.5cm} \tiny{89.54 - 147.93}  &\hspace{0.5cm} \tiny{$2.99_{-0.3}^{+0.2}$}	&\hspace{0.5cm}\tiny{$1.18_{-0.24}^{+0.26}$}	&\hspace{0.5cm}  \tiny{362/(16, 3)}&\hspace{0.5cm} \tiny{PL (-)}\\	

%\tiny{II}   	        & \hspace{0.5cm} \tiny{147.93 - 619.84}  &\hspace{0.5cm} \tiny{}&\hspace{0.5cm}  \tiny{$1.64_{-0.32}^{+0.34}$}	&\hspace{0.5cm}  \tiny{}&\\	

%\tiny{III}    	        & \hspace{0.5cm} \tiny{619.84 - 1570}  &\hspace{0.5cm} \tiny{$-2.82_{-0.20}^{+0.18}$}	&\hspace{0.5cm}\tiny{$1.19_{-0.24}^{+0.25}$}	&\hspace{0.5cm}  \tiny{16425/(449, 5)}&\hspace{0.5cm}  \tiny{SBPL ($1570_{-67}^{+68}$)}\\	&
%\hspace{0.5cm}\tiny{1570-$2.37 \times 10^{4}$} &   \hspace{0.5cm} \tiny{$1.43_{-0.05}^{+0.05}$}		&\hspace{0.5cm} \tiny{$1.02_{-0.09}^{+0.09}$} &\\	%\cdashline{}    
%
%\tiny{IV}    	        & \hspace{0.5cm} \tiny{$2.37 \times 10^{4}$ - $3.95 \times 10^{5}$} & \hspace{0.5cm} \tiny{$1.02_{-0.03}^{+0.03}$}&	\hspace{0.5cm} \tiny{$1.17_{-0.11}^{+0.07}$}	&\hspace{0.5cm}  \tiny{5053/(190, 5)}&\hspace{0.5cm}  \tiny{SBPL ($3.95_{-1.28}^{+2.39} \times 10^{5}$)} \\&	%
%\hspace{0.5cm} \tiny{$3.95 \times 10^{5}$ - $9.60 \times 10^{5}$}  &\hspace{0.5cm} \tiny{$1.33_{-0.29}^{+0.13}$}	&\hspace{0.5cm} \tiny{$1.33_{-0.24}^{+0.25}$}	&\\
%
%\tiny{V}   	        & \hspace{0.5cm} \tiny{$9.60 \times 10^{5}$ - $7.51 \times 10^{6}$}  &\hspace{0.5cm} \tiny{}	&\hspace{0.5cm}\tiny{$1.02_{-0.13}^{+0.28}$}	&\hspace{0.5cm}  \tiny{}&\hspace{0.5cm} \tiny{ (-)}\\
%\tiny{IV}   	        & \hspace{0.5cm} \tiny{619.84 - }  &\hspace{0.5cm} \tiny{}		&\hspace{0.5cm}  \tiny{$1.31$}\\
%\cdashline{}
%
%\tiny{III}   	        & \hspace{0.5cm} \tiny{$(0.25 - 26.1) \times10^4$ }  &\hspace{0.5cm} \tiny{$1.26\pm0.06$}		&\hspace{0.5cm}  \tiny{$1.29$}\\\cdashline{1-4}
%\tiny{IV}   	        & \hspace{0.5cm} \tiny{$\geq 2.6\times10^5$ }  &\hspace{0.5cm} \tiny{$1.75\pm0.09$}		&\hspace{0.5cm}  \tiny{$1.21$}\\
%
%\tiny{BPL}   	        &\hspace{0.5cm} \tiny{$1.24\pm0.08$} & \hspace{0.5cm} \tiny{$327.5\pm 25.3$}  &\hspace{0.5cm} \tiny{$1.28\pm0.06$}		&\hspace{0.5cm}  \tiny{$560/2163$}							                     \\
%\hline \hline
%\end{tabular}
%\end{table}
%
%








==> GRB 190829A arxiv22May/table_UVOT.tex <==
%\clearpage






\begin{table*}
\begin{scriptsize}
\begin{center}
\setlength{\tabcolsep}{2pt}

\caption{Log of UVOT observations $\&$ photometry of the GRB 190829A afterglow. No correction for galactic extinction is applied.}
\label{table:UVOT}
%\begin{tiny}

\begin{tabular}{@{}llllll@{}}
\toprule
Filter & $\rm T_{i}$ ($\rm s$) & $\rm T_{s}$ ($\rm s$) & Magnitude& Flux density ($\rm mJy$) \\ \hline
white & 106.3 & 256.1 & 19.51 $\pm$ 0.14 & 0.036 $\pm$ 0.005\\
white & 545.8 & 565.6 & 19.12 $\pm$ 0.29 & 0.051 $\pm$ 0.014\\
white & 721.6 & 741.3 & 18.87 $\pm$ 0.24 & 0.064 $\pm$ 0.014 \\
white & 870.6 & 1020.0 & 17.57 $\pm$ 0.04& 0.213 $\pm$ 0.008  \\
white & 1173.5 & 1366.5 & 16.88 $\pm$ 0.06& 0.401 $\pm$ 0.022 \\
white & 1519.3 & 1701.6 & 16.96 $\pm$ 0.08 & 0.373 $\pm$ 0.027 \\
white & 6079.3 & 6279.0 & 18.21 $\pm$ 0.05& 0.118 $\pm$ 0.005  \\
white & 10724.2 & 11631.1 & 18.85 $\pm$ 0.04& 0.065 $\pm$ 0.002 \\
white & 172223.6 & 173130.6 & 19.53 $\pm$ 0.06 & 0.035 $\pm$ 0.002 \\ \hline
b & 521.3 & 541.1 &  $>$ 18.76 & $>$ 0.127\\
b & 696.3 & 716.1 &  $>$ 18.76 & $>$ 0.127 \\
b & 1148.7 & 1342.2 & 17.24 $\pm$ 0.11& 0.516 $\pm$ 0.052  \\
b & 1495.0 & 1687.4 & 17.52 $\pm$ 0.16& 0.399 $\pm$ 0.059  \\
b & 5874.5 & 6074.3 & 18.43 $\pm$ 0.09& 0.172 $\pm$ 0.014 \\
b & 7310.3 & 7438.8 & 18.84 $\pm$ 0.30& 0.118 $\pm$ 0.032  \\
b & 99230.7 & 171611.5 & 19.80 $\pm$ 0.22 & 0.049 $\pm$ 0.010  \\
b & 171615.3 & 172218.5 & 19.54 $\pm$ 0.12& 0.062 $\pm$ 0.007 \\ \hline
u & 264.3 & 514.1 & 19.43 $\pm$ 0.23 & 0.025 $\pm$ 0.005 \\
u & 671.6 & 864.6 & 18.64 $\pm$ 0.34 & 0.052 $\pm$ 0.016  \\
u & 1123.8 & 1317.6  & 17.27 $\pm$ 0.16& 0.183 $\pm$ 0.027 \\
u & 1469.8 & 1662.5 & 17.77 $\pm$ 0.29& 0.115 $\pm$ 0.031  \\
u & 5669.3 & 5869.1 & 18.25 $\pm$ 0.11& 0.074 $\pm$ 0.007  \\
u & 7105.2 & 7304.9 & 18.56 $\pm$ 0.24& 0.056 $\pm$ 0.012  \\
u & 24564.2 & 24650.4 &  $>$ 18.40 & $>$  0.065\\
u & 98317.4 & 109397.7 & 19.35 $\pm$ 0.18& 0.027 $\pm$ 0.004  \\ 
u & 264490.8 & 271341.2 & 19.89 $\pm$ 0.22& 0.016 $\pm$ 0.003  \\\hline
v & 597.5 & 617.3 &  $>$ 17.72 &  $>$ 0.297 \\
v & 771.3 & 791.0 & 17.22 $\pm$ 0.27 & 0.471 $\pm$ 0.117  \\
v & 1050.3 & 1242.8 & 16.02 $\pm$ 0.10 & 1.421 $\pm$ 0.131   \\
v & 1396.2 & 1589.4 & 15.81 $\pm$ 0.10 & 1.724 $\pm$ 0.159   \\
v & 5054.5 & 5254.2 & 17.01 $\pm$ 0.08 & 0.571 $\pm$  0.042 \\
v & 6490.7 & 6690.4 & 17.36 $\pm$ 0.10 & 0.414 $\pm$ 0.038   \\
v & 17608.5 & 18515.3 & 18.49 $\pm$ 0.11 & 0.146 $\pm$ 0.015   \\
v & 45033.9 & 45941.0 & 18.59 $\pm$ 0.11 & 0.133 $\pm$ 0.013  \\
v & 167595.5 & 179056.0 & 18.82 $\pm$ 0.12 & 0.108 $\pm$ 0.012   \\ \hline
uvw1 & 647.4 & 1119.1 & 18.48 $\pm$ 0.36 & 0.040 $\pm$ 0.013   \\ 
uvw1 & 1273.5 & 1638.2 & $>$ 18.15 & $>$ 0.054\\
uvw1 & 5464.5 & 5664.2 & 19.26 $\pm$ 0.32 & 0.019 $\pm$ 0.006   \\
uvw1 & 6900.5 & 7100.3 & 18.99 $\pm$ 0.32 & 0.025 $\pm$ 0.007   \\
uvw1 & 23658.1 & 24557.8 & 19.74 $\pm$ 0.26 & 0.012 $\pm$ 0.003   \\
uvw1 & 87378.3 & 104975.0 & $>$ 20.48 & $>$ 0.006\\
uvw1 & 259190.3 & 270886.2 & 20.38 $\pm$ 0.33 & 0.007 $\pm$ 0.002   \\\hline
uvw2 & 4849.7 & 5049.5 & 19.19 $\pm$ 0.28 & 0.016 $\pm$ 0.004   \\
uvw2 & 6285.7 & 6485.5 & 19.11 $\pm$ 0.28 & 0.017 $\pm$  0.004 \\
uvw2 & 11637.3 & 12112.8 & 20.01 $\pm$ 0.33 & 0.007 $\pm$ 0.002   \\
uvw2 & 27922.6 & 30389.2 & 19.71 $\pm$ 0.29 & 0.010 $\pm$ 0.003   \\
uvw2 & 33673.8 & 40012.9 & 20.14 $\pm$ 0.26 & 0.007 $\pm$ 0.002  \\
uvw2 & 166688.4 & 173821.9 & $>$ 20.62 & $>$ 0.004 \\ \hline
uvm2 & 5259.3 & 5459.1 & $>$ 19.33 &  $>$ 0.014 \\
uvm2 & 6695.5 & 6895.2 & $>$ 19.22 &  $>$ 0.016  \\
uvm2 & 18520.3 & 18914.0 & $>$ 19.63 &  $>$ 0.011  \\
uvm2 & 22751.2 & 23651.0 & 20.39 $\pm$ 0.36 & 0.005 $\pm$ 0.002   \\
uvm2 & 86471.6 & 103671.5 & 20.00 $\pm$ 0.19 & 0.008 $\pm$ 0.001   \\
uvm2 & 179061.3 & 259183.4 & 20.17 $\pm$ 0.29 & 0.007 $\pm$  0.002 \\
uvm2 & 269079.1 & 269978.9 & 20.38 $\pm$ 0.34 & 0.005 $\pm$ 0.002 \\\hline
\end{tabular}
 \end{center}

\end{scriptsize}
\end{table*}


==> GRB 190829A arxiv22May/table_lag.tex <==
\begin{table*}
\begin{center}
\caption{ Time lag w.r.t 150-300 keV photons label{lag_table}}
\begin{tabular}{c|c|c}
\hline
- & Episode-1 & Episode-2 \\
\hline
Energy Band & Lag(Correlation) & Lag(Correlation) \\
(keV) & (sec(\%)) & (sec(\%)) \\
\hline
\multicolumn{5}{c}{4ms timebin} \\
\hline
8-30 & $1.135\pm0.006(6.38\pm0.01)$ & $0.462\pm0.006(11.67\pm0.00)$ \\
30-50 & $0.848\pm0.006(4.84\pm0.01)$ & $0.618\pm0.021(8.49\pm0.00)$ \\
50-100 & $0.086\pm0.008(3.81\pm0.01)$ & $-0.047\pm0.003(4.59\pm0.01)$ \\
8-100 & $0.723\pm0.016(8.21\pm0.04)$ & $0.619\pm0.025(11.82\pm0.00)$ \\
\hline
\multicolumn{5}{c}{8ms timebin} \\
\hline
8-30 & $0.071\pm0.003(63.01\pm0.01)$ & $0.100\pm0.004(64.97\pm0.01)$ \\
30-50 & $-0.003\pm0.003(58.51\pm0.02)$ & $-0.042\pm0.005(60.96\pm0.01)$ \\
50-100 & $0.051\pm0.003(56.91\pm0.02)$ & $-0.083\pm0.002(56.89\pm0.02)$ \\
8-100 & $0.081\pm0.002(66.17\pm0.01)$ & $0.040\pm0.003(65.94\pm0.01)$ \\
\hline
\multicolumn{5}{c}{16ms timebin} \\
\hline
8-30 & $1.215\pm0.007(11.43\pm0.01)$ & $0.528\pm0.097(16.72\pm0.02)$ \\
30-50 & $0.717\pm0.008(8.98\pm0.01)$ & $0.454\pm0.038(13.82\pm0.01)$ \\
50-100 & $0.156\pm0.008(7.32\pm0.02)$ & $-0.048\pm0.004(8.40\pm0.01)$ \\
8-100 & $0.755\pm0.007(14.09\pm0.10)$ & $0.533\pm0.109(16.84\pm0.01)$ \\
\hline
\end{tabular}
\end{center}
\end{table*}


==> GRB 190829A arxiv22May/table_tr.tex <==
\begin{table*}[!h]
\caption{Time-resolved spectral fitting of prompt emission Episode 1 \& Episode 2 (\fermi-GBM) and spectral fitting of the afterglow phases.}
\setlength{\tabcolsep}{2pt}
%\begin{left}
\flushleft
\begin{center}
\footnotesize
    Prompt Emission Episode 1
\end{center}
\begin{tiny}
\setlength\tabcolsep{1.0pt} 
\begin{tabular}{|p{1.45cm}|p{1.7cm}p{1.7cm}|p{1.7cm}p{1.7cm}p{1.7cm}|p{1.7cm}p{1.72cm}p{1.75cm}p{1.75cm}|p{1.75cm}p{1.75cm}p{1.75cm}|}
%\begin{tabular}{\linewidth}{@{\extracolsep{\fill}}lllllllllllll}
\cline{1-10}
%\multicolumn{10}{|l|}{Prompt Emission Episode 1} \\
%\cline{1-10}
\cline{1-10}
 \multicolumn{1}{|c|}{Time (s)} & \multicolumn{2}{c|}{PL} & \multicolumn{3}{c|}{COMP} & \multicolumn{4}{c|}{Band}  &\\
%  \multicolumn{3}{c}{BBPL} \\
\cline{2-10}
 $\rm $ & $\rm \alpha$ & \sw{pgstat}(BIC) & $\rm \alpha$ & $\rm E_{p}$ $\rm (keV)$ & \sw{pgstat}(BIC) & $\rm \alpha$ & $\rm \beta$ & $\rm E_{p}$ $\rm (keV)$ & \sw{pgstat}(BIC) \\ 
  &  & dof = $\rm 467$ &  &  &  dof = $\rm 466$ &  &  &  & dof = $\rm 465$ \\ 
 \cline{1-10}
 -0.64 - 0.85 & $1.49_{-0.05}^{+0.06}$ & $463.6(494.4)$ & $1.14_{-0.21}^{+0.19}$    & $311_{-112}^{+324}$ & $453.5(490.5)$ & $-1.01_{-0.28}^{+0.36}$ & $-1.89_{+1.89}^{+0.26}$ & $194_{-84}^{+314}$ & $452.3(495.4)$ \\
 0.85 - 1.64  & $1.63_{-0.07}^{+0.08}$ & $490.8(521.6)$ & $1.26_{-0.31}^{+0.27}$    & $155_{-52}^{+279}$  & $484.2(521.1)$ & $-0.75_{-0.64}^{+0.75}$ & $-1.88_{-0.95}^{+0.19}$ & $65_{-35}^{+132}$  & $480.8(523.9)$ \\
 1.64 - 2.72  & $1.78_{-0.08}^{+0.08}$ & $532.9(563.7)$ & $1.22_{-0.33}^{+0.28}$    & $86_{-19}^{+42}$    & $517.1(554.0)$ & $-1.07_{-0.32}^{+0.72}$ & $-2.46_{+2.46}^{+0.45}$ & $71_{-30}^{+38}$   & $516.3(559.4)$ \\
 2.72 - 3.96  & $1.87_{-0.09}^{+0.10}$ & $480.0(510.8)$ & $1.43_{-0.40}^{+0.34}$    & $68_{-18}^{+66}$    & $474.6(511.6)$ & $-1.20_{-0.46}^{+0.66}$ & $-2.30_{+2.30}^{+0.32}$ & $52_{-17}^{+41}$   & $472.8(515.9)$ \\
 3.96 - 8.06  & $2.18_{-0.12}^{+0.14}$ & $540.8(571.6)$ & $1.83_{-0.45}^{+\infty}$  & $21_{-16}^{+18}$    & $537.2(574.2)$ & $-0.43_{-1.99}^{+0.43}$ & $-2.34_{+2.34}^{+0.20}$ & $19_{-6}^{+18}$    & $536.5(579.6)$ \\
 \cline{1-10}
\end{tabular}
\end{tiny}
%\end{left}


\begin{center}
\footnotesize
    Prompt Emission Episode 2
\end{center}
\begin{tiny}
%\begin{left}

\begin{tabular}{|l|ll|lll|llll|lll|}
\hline
%\multicolumn{13}{|l|}{Prompt Emission Episode 2} \\
%\hline
%\hline

\multicolumn{1}{|c|}{Time (s)} &\multicolumn{2}{c|}{PL} & \multicolumn{3}{c|}{CPL} & \multicolumn{4}{c|}{Band} & \multicolumn{3}{c|}{BB+PL}\\
\cline{2-13}
& $\rm \alpha$ & \sw{pgstat}(BIC) & $\rm \alpha$ & $\rm E_{c}$ $\rm (keV)$ & \sw{pgstat}(BIC) & $\rm \alpha$ & $\rm \beta$ & $\rm E_{ p}$ $\rm (keV)$ & \sw{pgstat}(BIC) & $\rm \alpha$ & kT $\rm (keV)$ & \sw{pgstat}(BIC)\\ 
  &  & dof= $\rm 450$ &  &  & dof= $\rm 449$ &  &  &  & dof = $\rm 448$ & & & dof = $\rm 448$\\
\hline

47.04 - 49.03 & $2.31_{-0.06}^{+0.06}$ & $452.4(483.0)$ & $2.12_{-0.15}^{+0.14}$ & $240_{-115}^{+605}        	  $  & $446.1(482.8)$ & $  0.75_{-0.95}^{+\infty}  $ & $ -2.38_{-0.06}^{+0.05} $ & $ 14.02_{-0.18}^{+1.44}   $  & $442.6(485.5) $ & $ 2.20_{-0.12}^{+0.11} $ & $ 4.2_{-0.8}^{+1.7}    $ & $ 446.9(489.7) $\\
49.03 - 49.68 & $2.48_{-0.06}^{+0.06}$ & $471.3(501.9)$ & $2.27_{-0.17}^{+0.18}$ & $182_{-85}^{+745}      $  & $466.3(503.0)$ & $ -1.00_{-1.12}^{+1.00}    $ & $ -2.57_{-0.25}^{+0.08} $ & $ 12.29_{-5.17}^{+2.18}   $  & $462.0(504.8) $ & $ 2.43_{-0.12}^{+0.12} $ & $ 5.0_{-1.3}^{+4.2}    $ & $ 464.6(507.4) $\\
49.68 - 50.21 & $2.43_{-0.06}^{+0.06}$ & $573.2(603.8)$ & $2.41_{-0.13}^{+0.07}$ & $2278_{-1967}^{+\infty}      $  & $573.1(609.8)$ & $  0.98_{-0.98}^{+\infty}  $ & $ -2.44_{-0.06}^{+0.06} $ & $ 10.49_{-0.11}^{+1.74}   $  & $571.5(614.4) $ & $ 2.39_{-0.13}^{+0.15} $ & $ 4.4_{-4.4}^{+5.6}    $ & $ 572.0(614.9) $\\
50.21 - 50.66 & $2.46_{-0.05}^{+0.06}$ & $400.1(430.6)$ & $2.33_{-0.16}^{+0.14}$ & $328_{-185}^{+6799}          $  & $397.0(433.6)$ & $  1.00_{-1.00}^{+\infty}  $ & $ -2.51_{-0.07}^{+0.07} $ & $ 11.94_{-0.17}^{+1.42}   $  & $392.4(435.3) $ & $ 2.38_{-0.12}^{+0.15} $ & $ 3.4_{-2.4}^{+\infty} $ & $ 398.0(440.8) $\\
50.66 - 51.11 & $2.50_{-0.06}^{+0.06}$ & $501.3(531.9)$ & $2.50_{-0.08}^{+0.04}$ & ---    & $501.3(538.1)$ & $  0.96_{-0.96}^{+\infty}  $ & $ -2.51_{-0.04}^{+0.04} $ & $  9.44_{-0.10}^{+1.99}   $  & $501.0(543.6) $ & $ 2.34_{-0.14}^{+0.14} $ & $ 2.9_{-0.8}^{+0.6}    $ & $ 497.0(539.5) $\\
51.11 - 51.52 & $2.40_{-0.05}^{+0.06}$ & $488.0(518.2)$ & $2.26_{-0.16}^{+0.14}$ & $299_{-164}^{+3034}          $  & $484.0(520.8)$ & $ -1.36_{-0.50}^{+1.36}    $ & $ -2.52_{-0.11}^{+0.09} $ & $ 13.41_{-8.05}^{+3.06}   $  & $475.2(518.0) $ & $ 2.30_{-0.12}^{+0.10} $ & $ 4.8_{-0.8}^{+1.6}    $ & $ 475.0(517.9) $\\
51.52 - 51.93 & $2.44_{-0.05}^{+0.06}$ & $497.8(528.4)$ & $2.40_{-0.13}^{+0.09}$ & $1324_{-1048}^{+\infty}      $  & $497.4(534.1)$ & $ -1.81_{-0.65}^{+1.81}    $ & $ -2.49_{-0.10}^{+0.08} $ & $  5.92_{-2.46}^{+7.44}   $  & $495.0(537.8) $ & $ 2.34_{-0.13}^{+0.11} $ & $ 4.1_{-0.8}^{+1.7}    $ & $ 493.0(535.8) $\\
51.93 - 52.37 & $2.44_{-0.06}^{+0.05}$ & $515.1(545.7)$ & $2.44_{-0.10}^{+0.04}$ & ---   & $515.1(551.8)$ & $  0.98_{-0.80}^{+\infty}  $ & $ -2.48_{-0.07}^{+0.07} $ & $ 12.07_{-0.13}^{+1.48}   $  & $508.4(551.2) $ & $ 2.22_{-0.15}^{+0.13} $ & $ 3.7_{-0.4}^{+0.5}    $ & $ 503.0(545.8) $\\
52.37 - 52.80 & $2.47_{-0.06}^{+0.06}$ & $431.6(462.2)$ & $2.34_{-0.16}^{+0.14}$ & $315_{-174}^{+5454}       	  $  & $428.5(465.3)$ & $  0.91_{-1.49}^{+\infty}  $ & $ -2.52_{-0.05}^{+0.05} $ & $ 12.05_{-0.13}^{+1.50}   $  & $425.9(468.7) $ & $ 2.40_{-0.13}^{+0.06} $ & $ 4.1_{-1.0}^{+3.9}    $ & $ 428.3(471.1) $\\
52.80 - 53.26 & $2.46_{-0.06}^{+0.06}$ & $501.8(532.4)$ & $2.36_{-0.15}^{+0.14}$ & $393_{-237}^{+\infty}        $  & $500.0(536.7)$ & $  1.00_{-10.95}^{+\infty} $ & $ -2.52_{-0.08}^{+0.07} $ & $ 12.37_{-0.14}^{+1.49}   $  & $494.8(537.7) $ & $ 2.32_{-0.13}^{+0.13} $ & $ 3.6_{-0.6}^{+1.0}    $ & $ 496.4(539.2) $\\
53.26 - 53.77 & $2.47_{-0.05}^{+0.06}$ & $453.8(484.4)$ & $2.39_{-0.13}^{+0.11}$ & $568_{-366}^{+\infty}        $  & $452.1(488.8)$ & $ -2.05_{-\infty}^{+2.05}  $ & $ -2.50_{-0.08}^{+0.07} $ & $  10.39_{-\infty}^{+2.33} $  & $454.0(496.6) $ & $ 2.42_{-0.12}^{+0.17} $ & $ 4.0_{-4.0}^{+\infty}  $ & $ 452.6(495.5) $\\
53.77 - 54.39 & $2.53_{-0.06}^{+0.06}$ & $481.2(511.8)$ & $2.47_{-0.16}^{+0.11}$ & $682_{-503}^{+\infty}        $  & $481.0(517.5)$ & $ -1.63_{-0.87}^{+1.63}    $ & $ -2.63_{-0.11}^{+0.09} $ & $  8.16_{-5.08}^{+5.40}   $  & $474.0(516.8) $ & $ 2.38_{-0.15}^{+0.13} $ & $ 4.0_{-0.5}^{+1.0}    $ & $ 470.6(513.4) $\\
54.39 - 55.08 & $2.56_{-0.06}^{+0.07}$ & $419.0(448.7)$ & $2.52_{-0.19}^{+0.11}$ & $739_{-592}^{+\infty}        $  & $417.7(454.4)$ & $ -1.13_{-2.15}^{+1.13}    $ & $ -2.64_{-0.15}^{+0.09} $ & $ 10.00_{-4.19}^{+2.96}   $  & $413.7(456.5) $ & $ 2.47_{-0.17}^{+0.13} $ & $ 4.0_{-0.7}^{+1.9}    $ & $ 412.3(455.2) $\\
55.08 - 56.02 & $2.55_{-0.07}^{+0.06}$ & $517.2(547.8)$ & $2.53_{-0.17}^{+0.06}$ & $3607_{-3402}^{+\infty}      $  & $517.2(553.9)$ & $  0.99_{-0.79}^{+\infty}  $ & $ -2.60_{-0.09}^{+0.08} $ & $ 11.53_{-0.12}^{+1.38}   $  & $511.4(554.3) $ & $ 2.41_{-0.17}^{+0.14} $ & $ 3.5_{-0.6}^{+1.4}    $ & $ 513.0(554.9) $\\
56.02 - 57.50 & $2.55_{-0.07}^{+0.07}$ & $498.3(528.9)$ & $2.55_{-0.12}^{+0.07}$ & ---  & $498.3(535.0)$ & $ -0.40_{-3.13}^{+0.40}    $ & $ -2.61_{-0.10}^{+0.08} $ & $ 10.71_{-2.81}^{+1.85}   $  & $494.4(537.2) $ & $ 2.29_{-0.17}^{+0.17} $ & $ 3.3_{-0.4}^{+0.4}    $ & $ 487.4(530.2) $\\
57.50 - 62.46 & $2.64_{-0.08}^{+0.09}$ & $507.1(537.7)$ & $2.64_{-0.10}^{+0.08}$ & --- & $507.1(543.8)$ & $  0.95_{-3.44}^{+\infty} $ & $-2.70_{-0.08}^{+0.07}$ & $10.44_{-0.12}^{+1.45}$  & $504.0(546.8)$ & $2.16_{-0.21}^{+0.21}$ & $2.9_{-0.3}^{+0.2}$ & $488.3(531.1)$ \\ \hline
\end{tabular}
%\end{left}
\end{tiny}

\begin{center}
\footnotesize
    Afterglow
\end{center}
\begin{tiny}
%\begin{left}
\begin{tabular}{|p{3.0cm}|p{1.65cm}|p{4.468cm}p{4.468cm}p{4.05cm}|}
\hline
%\multicolumn{5}{|l|}{Afterglow} 
%\cline{1-5}
\cline{1-5}
\multicolumn{1}{|c|}{(Phase) Time (s) }&
\multicolumn{1}{c|}{Detectors}&
\multicolumn{3}{c|}{\sw{Tbabs*zTBabs*cflux}*PL}  \\
\cline{3-5}
  & & $n_{H}$ &$\rm \alpha$ & \sw{Statistics}(BIC) \\
\cline{1-5}
(I) 104-228 & XRT +BAT & $0.84_{-0.20}^{+0.27}$ & $2.11_{-0.17}^{+0.20}$& 125.1/103  \\
(IV-pre-break)  23.7k - 167k & XRT   &  $1.03_{-0.12}^{+0.13}$ &  $2.02_{-0.11}^{+0.12}$ &532.1/541   \\
(IV post-break) 167k - 1550k & XRT   &  $1.12_{-0.12}^{+0.13}$ &  $2.35_{-0.13}^{+0.13}$ &  486.76/489      \\
\hline
\end{tabular}
%\end{left}
%\begin{left}
\begin{tabular}{|p{3.0cm}|p{1.65cm}|llll|lllllp{1.1cm}|}
\hline
 \multicolumn{1}{|c|}{(Phase) Time (s) } &
 \multicolumn{1}{c|}{Detectors}&
 \multicolumn{4}{c|}{\sw{redden*phabs*zdust}*PL}& \multicolumn{6}{c|}{\sw{redden*phabs*zdust}*\sw{bknpower}} \\
\cline{3-12}
& & $ \rm n_{H}$ &$\rm \Gamma$ & \sw{Statistics}(BIC) & $\rm E_{B-V}$ & $n_{H}$ & $\rm \Gamma_1$ & $\rm \Gamma_2$ & $\rm E_b$ & \sw{Statistics}(BIC) & $\rm E_{B-V}$  \\
\cline{1-12}
 
(III-pre) 147 - 620  & UVOT + XRT     & $0.86_{-0.20}^{+0.23}$ & $1.84_{-0.15}^{+0.14}$& 39.7/26 &$1.14_{-0.28}^{+0.25}$ 
& $0.80_{-0.38}^{+0.32}$ & $1.50_{-0.54}^{+0.29}$  & $3.14_{-0.44}^{+0.85}$ & $3.54_{-0.89}^{+3.54}$& 25.9/24& $0.67_{-0.63}^{+0.43}$  \\
(III-rise)  620 - 1120 & UVOT + XRT     & $1.26_{-0.23}^{+0.33}$ & $1.92_{-0.12}^{+0.21}$ &56.5/30&$1.08_{-0.25}^{+0.48}$
-- & -- &    --    & -- & --  & -- & --            \\
(III-top)  1120-1700  & UVOT + XRT   & $1.41_{-0.07}^{+0.07}$ & $1.99_{-0.04}^{+0.05}$ &404.3/353&$1.33_{-0.10}^{+0.11}$     & $1.36_{-0.07}^{+0.07}$ & $1.84_{-0.06}^{+0.07}$  & $2.59_{-0.55}^{+0.81}$& $2.15_{-0.09}^{+0.17}$  &378.9/351  & $1.04_{-0.12}^{+0.14}$  \\
\cline{1-12}
\end{tabular}
%\end{left}

%\begin{tabular}{|l|l|l|lll|ll|}
%\hline
%\multicolumn{5}{|l|}{Afterglow} \\
%\cline{1-5}
%\cline{1-5}
%\multicolumn{1}{c|}{Phase} &
%\multicolumn{1}{|c|}{(Phase) Time} & %\multicolumn{1}{c|}{Detectors} & 
%\multicolumn{4}{c}{\sw{Tbabs*zTBabs*cflux}* PL} & %\multicolumn{1}{c|}{} & %\multicolumn{1}{c|}{} \\
%\cline{1-5}
% $\rm (s)$ & $\rm N_{H} (z)$ &  $\rm \Gamma$ ($\rm \Gamma_{1}$, $\rm \Gamma_{2}$) & Statistics$^a$ &\\
%\cline{1-5}
% (I) 104-228  & XRT (WT) & PL &      $0.76^{+0.22}_{-0.17}$ & $2.12_{-0.18}^{+0.20}$ & -- &390.3/383 \\
 
%& &   CPL      & $0.12_{-0.12}^{+0.20}$  & $-0.63_{-0.73}^{+0.81}$ & $1.12_{-0.27}^{+0.50}$& 357.4/382   \\
%&  &   BB + PL &    $0.04_{-0.04}^{+0.09}$  &$0.71_{-0.31}^{+0.52}$ & -- & $0.69^{+0.05}_{-0.05}$& --&354.5/382\\ 
%(I) 104-228 & $0.84_{-0.20}^{+0.27}$ & $2.11_{-0.17}^{+0.20}$& 125.1/103 &  \\
%&  &  CPL &      $0.15^{+0.24}_{-0.16}$   & $-0.49^{+0.86}_{-0.81}$ & $1.21_{-0.32}^{+0.65}$&  103.7/102  \\ \hline
%& &   \sw{bknpow}       & $1.27_{-0.15}^{+0.16}$ & $2.59_{-0.16}^{+0.18}$  & $4.93_{-0.72}^{+0.60}$ & 465.9/487 &--              \\  
%&  &        &  & $0.40_{-1.04}^{+0.87}$  &  &  & &                \\ \hline
%(III pre)  147 - 620  & XRT (WT $\&$ PC) & PL    & $1.59_{-0.27}^{+0.31}$ & $2.46_{-0.22}^{+0.23}$& 494.3/548    &           \\%\hline
%& &   \sw{bknpow}       & $1.12_{-0.42}^{+0.21}$ & $1.77_{-0.73}^{+0.48}$  & $2.89_{-0.48}^{+0.62}$ & 486.0/546               \\  &  &        &  & $3.00_{-0.36}^{+0.60}$  &  &  & \\ 
%(III-rise) 620 - 1140 & XRT (WT $\&$ PC) & PL    & $1.44_{-0.26}^{+0.29}$ & $2.18_{-0.21}^{+0.22}$& 583.8/554   &            \\%\hline
%& &   \sw{bknpow}       & $1.45_{-0.18}^{+0.26}$ & $2.20_{-2.23}^{+\infty}$  & $0.48_{-0.08}^{+\infty}$ & 584/552              \\  &  &        &  & $2.20_{-0.21}^{+0.22}$  &  &              \\               
%(III-top)  1120-1700 & XRT (WT) & PL    & $1.42_{-0.08}^{+0.08}$ & $2.03_{-0.06}^{+0.06}$ &823.9/758      &         \\
%& &   \sw{bknpow}       & $0.76_{-0.21}^{+0.22}$ & $0.63_{-0.51}^{+0.50}$  & $1.81_{-0.09}^{+0.15}$ & 796.2/756              \\  &  &        &  & $1.96_{-0.07}^{+0.08}$  &  &  &                \\ 
%(III-decay)  4860-23700 & XRT (PC) & PL    & $1.25_{-0.11}^{+0.12}$ & $2.01_{-0.09}^{+0.09}$&554.3/603   & \\
%(IV-pre-break)  23700 - 167000    &  $1.03_{-0.12}^{+0.13}$ &  $2.02_{-0.11}^{+0.12}$ &532.1/541        &   \\
%(IV post-break) 167000 - 1550000     &  $1.12_{-0.12}^{+0.13}$ &  $2.35_{-0.13}^{+0.13}$ &  486.76/489    &          \\
%& &   \sw{bknpow}       & $1.07_{-0.21}^{+0.20}$ & $1.68_{-0.44}^{+0.30}$  & $2.46_{-0.38}^{+1.01}$ & 550.2/601               \\  &  &        &  & $2.11_{-0.13}^{+0.19}$  &    &&               \\ \hline
% \hline
%(s) & &  \sw{redden*phabs*zdust*} & $\rm N_{H} (z)$ & $\rm \Gamma$ ($\rm \Gamma_{1}$, $\rm \Gamma_{2}$) & $\rm  E_{b}$ & $\chi^{2}$/dof & $\rm E_{B-V} $  \\
 %& &\sw{zphabs*}   &    &  &                     &  & \\
%(III-decay)  4860-23700     & $0.96_{-0.06}^{+0.06}$ & $1.69_{-0.02}^{+0.03}$ &171.2/147 &$0.56_{-0.04}^{+0.05}$ & $1.11_{-0.08}^{+0.10}$ & $1.64_{-0.03}^{+0.03}$ &$2.26_{-0.46}^{+0.63}$ & $2.10_{-0.12}^{+0.19}$  &125.2/145 & $0.52_{-0.04}^{+0.04}$\\
%\hline
%(III-pre) 147 - 620       & $0.86_{-0.20}^{+0.23}$ & $1.84_{-0.15}^{+0.14}$& -- &39.7/26 &$1.14_{-0.28}^{+0.25}$               \\
%&  &   \sw{bknpow}       & $0.80_{-0.38}^{+0.32}$ & $1.50_{-0.54}^{+0.29}$  & $3.14_{-0.44}^{+0.85}$ &  25.9/24& $0.67_{-0.63}^{+0.43}$              \\
% &  & & &$3.54_{-0.89}^{+3.54}$  &  &  &              \\ %\hline
%(III-rise)  620 - 1120      & $1.26_{-0.23}^{+0.33}$ & $1.92_{-0.12}^{+0.21}$& -- &56.5/30&$1.08_{-0.25}^{+0.48}$              \\
%&  & \sw{bknpow}       & 1.28 & 1.94  & 18.73  & 56.4/28&1.11               \\ 
% &  &        &  & 2.30  &  &  &             \\ %\hline
%(III-top)  1120-1700     & $1.41_{-0.07}^{+0.07}$ & $1.99_{-0.04}^{+0.05}$& -- &404.3/353&$1.33_{-0.10}^{+0.11}$               \\
%&   & \sw{bknpow}       & $1.36_{-0.07}^{+0.07}$ & $1.84_{-0.06}^{+0.07}$  & $2.59_{-0.55}^{+0.81}$ &378.9/351  & $1.04_{-0.12}^{+0.14}$             \\ 
% &  &        &  & $2.15_{-0.09}^{+0.17}$  &  &  &                \\ 
%(III-decay)  4860-23700     & $0.96_{-0.06}^{+0.06}$ & $1.69_{-0.02}^{+0.03}$ &-- &171.2/147 &$0.56_{-0.04}^{+0.05}$  \\
%&   & \sw{bknpow}       & $1.11_{-0.08}^{+0.10}$ & $1.64_{-0.03}^{+0.03}$ &$2.26_{-0.46}^{+0.63}$ &125.2/145 & $0.52_{-0.04}^{+0.04}$          \\ 
% &          &  & & $2.10_{-0.12}^{+0.19}$  &  &  &     \\ 
%\hline
%\end{tabular}
%\vspace{2cm}
$a$: $\chi^2$/dof for joint BAT-XRT data and UVOT-XRT data and \sw{C-stat} for XRT data. All errors are quoted at $1 \sigma$ (nominal 68\%) confindence level.
 $\rm N_{H} (z)$ : in units of $\rm 10^{22}$ $\rm cm^{-2}$;
$\rm  E_{b}$ are the break and cutoff energies, respectively in $\rm keV$. Reddening parameter in host is obtained for SMC extinction law. 
\end{tiny}
\label{tab:tr_spectral}
\end{table*}




==> GRB 190829A arxiv22May/table_two_episodes.tex <==
%Tables

\clearpage
\begin{table*}%
\caption{Bursts with two-episode emission and redshift detection}
\setlength{\tabcolsep}{2pt}

\begin{scriptsize}
\begin{center}
\begin{tabular}{ccccccccccc}
\\
\hline
\\
Trigger ID& z & $\rm T_{Ep.,1}$,   &    & $\rm F_{Ep.,1}$  & $\rm F_{peak,1}$ & $\rm E_{p,1}$ & $\rm \alpha_{1}$  & $\rm E_{iso, 1}$ & $\rm L_{iso,1}$ & Model$\rm _{Ep.,1}$  \\ 

&  &  $\rm T_{Ep.,2}$ & $\rm T_{q}$ & $\rm F_{Ep.,2}$ & $\rm F_{peak,2}$ & $\rm E_{p,2}$ & $\rm \alpha_{2}$ & $\rm E_{iso,2}$ & $\rm L_{iso,2}$ & Model$\rm _{Ep.,2}$ \\

&  &  ($\rm s$)  & ($\rm s$) & &    & ($\rm keV$) &  &  & &  \\

\hline
bn090328401 &$0.736$&$36.68$&--&$1.949_{-0.138}^{+0.136}$& $4.290_{-0.287}^{+0.862}$ &$655_{-65}^{+78}    $&$-0.96_{-0.03}^{+0.03}  $&$ 10.62   $&$  1.054 $& Band  \\ & &$ 18.36 $&$ 13.31 $&$ 0.117_{-0.014}^{+0.018} $& $0.410_{-0.104}^{+0.092}$  &$  96_{-17}^{+32}   $&$+1.26_{-0.21}^{+0.19}  $&$   0.37 $&$ 0.101  $& COMP   \\
\hline
bn091208410 &$1.063$&$ 4.33$&--&$0.392_{-0.041}^{+0.051}$& $0.751_{-0.105}^{+0.153}$ &$102_{-17}^{+28}    $&$+1.19_{-0.19}^{+0.17}  $&$  4.27   $&$  0.461 $& COMP  \\ & &$  5.85 $&$  3.58 $&$ 0.656_{-0.045}^{+0.052} $& $2.381_{-0.167}^{+0.193}$  &$ 129_{-15}^{+20}   $&$+1.15_{-0.10}^{+0.10}  $&$   1.14 $&$ 1.461  $& COMP   \\
\hline
bn100615083 &$1.398$&$25.51$&--&$0.369_{-0.066}^{+0.084}$& $0.869_{-0.184}^{+0.209}$ &$ 86_{-31}^{+18}    $&$-1.10_{-0.13}^{+0.29}  $&$  0.89   $&$  1.058 $& Band  \\ & &$ 18.37 $&$  3.07 $&$ 0.130_{-0.013}^{+0.016} $& $0.264_{-0.047}^{+0.062}$  &$  72_{-11}^{+17}   $&$-1.35_{-0.18}^{+0.16}  $&$   1.21 $&$ 0.321  $& COMP   \\ 
\hline
bn111228657 &$0.714$&$37.76$&--&$0.259_{-0.024}^{+0.027}$& $1.705_{-0.197}^{+0.268}$ &$ 48_{-4}^{+4}      $&$-1.63_{-0.07}^{+0.07}  $&$  1.01   $&$  0.389 $& Band  \\ & &$ 20.39 $&$ 19.46 $&$ 0.284_{-0.017}^{+0.017} $& $0.830_{-0.051}^{+0.095}$  &$  15_{-1}^{+1}     $&$+0.41_{-1.35}^{+3.70}$&$   0.84 $&$ 0.189  $& Band  \\
\hline
bn120711115 &$1.405$&$10.20$&--&$0.354_{-0.104}^{+0.163}$& $1.079_{-0.381}^{+0.982}$ &$389_{-131}^{+278}  $&$+0.41_{-0.62}^{+0.42}  $&$  6.85   $&$  1.329 $& COMP  \\ & &$ 65.16 $&$ 50.18 $&$ 5.160_{-0.133}^{+0.105} $& $15.075_{-1.607}^{+1.842}$ &$1123_{-88}^{+58}   $&$-0.95_{-0.01}^{+0.02}  $&$ 172.27 $&$18.576  $& Band   \\
\hline
bn120716712 &$2.486$&$ 7.14$&--&$0.236_{-0.036}^{+0.051}$& $0.957_{-0.123}^{+0.125}$ &$152_{-37}^{+74}    $&$+1.10_{-0.26}^{+0.21}  $&$  3.49   $&$  4.841 $& COMP  \\ & &$ 47.95 $&$169.47 $&$ 0.263_{-0.024}^{+0.034} $& $0.568_{-0.046}^{+0.085}$  &$ 113_{-11}^{+10}   $&$-0.87_{-0.09}^{+0.11}  $&$  18.30 $&$ 2.873  $& Band   \\
\hline
bn131108024 &$2.400$&$12.24$&--&$0.236_{-0.024}^{+0.031}$& $0.868_{-0.129}^{+0.161}$ &$132_{-22}^{+34}    $&$+1.03_{-0.19}^{+0.17}  $&$  2.30   $&$  4.028 $& COMP  \\ & &$ 54.09 $&$219.13 $&$ 0.176_{-0.035}^{+0.084} $& $0.403_{-0.112}^{+0.250}$  &$ 410_{-139}^{+133} $&$-0.46_{-0.23}^{+0.35}  $&$  24.44 $&$ 1.870  $& Band   \\
\hline
bn140304849 &$5.283$&$36.74$&--&$0.146_{-0.038}^{+0.034}$& $0.404_{-0.100}^{+0.160}$ &$548_{-307}^{+1043} $&$+1.41_{-0.19}^{+0.13}  $&$  8.78   $&$ 12.476 $& COMP  \\ & &$ 70.40 $&$148.48 $&$ 0.084_{-0.008}^{+0.009} $& $0.333_{-0.069}^{+0.091}$  &$  94_{-13}^{+18}   $&$+1.03_{-0.16}^{+0.18}  $&$  29.07 $&$10.284  $& COMP   \\
\hline
bn140512814 &$0.725$&$13.25$&--&$0.756_{-0.103}^{+0.121}$& $2.297_{-0.648}^{+0.710}$ &$627_{-192}^{+344}  $&$+1.09_{-0.07}^{+0.06}  $&$  3.81   $&$  0.544 $& COMP  \\ & &$ 67.27 $&$ 83.97 $&$ 0.555_{-0.045}^{+0.054} $& $2.941_{-0.516}^{+0.778}$  &$ 436_{-59}^{+78}   $&$+1.16_{-0.04}^{+0.04}  $&$   5.12 $&$ 0.696  $& COMP   \\
\hline
bn151027166 &$0.810$&$25.50$&--&$0.209_{-0.016}^{+0.021}$& $1.125_{-0.098}^{+0.097}$ &$135_{-20}^{+29}    $&$+1.31_{-0.11}^{+0.11}  $&$  1.32   $&$  0.351 $& COMP  \\ & &$ 31.62 $&$ 71.68 $&$ 0.497_{-0.078}^{+0.092} $& $1.270_{-0.349}^{+0.631}$  &$ 538_{-173}^{+271} $&$+1.42_{-0.07}^{+0.05}  $&$   2.71 $&$ 0.396  $& COMP   \\
\hline
bn180728728 &$0.117$&$ 4.08$&--&$0.313_{-0.041}^{+0.044}$& $0.536_{-0.091}^{+0.081}$ &$ 14_{-4}^{+2}      $&$+0.21_{-1.98}^{+\infty}$&$  0.02   $&$  0.002 $& Band  \\ & &$  9.02 $&$  7.17 $&$ 6.392_{-0.010}^{+0.012} $& $19.794_{-0.501}^{+0.522}$ &$  81_{-1}^{+1}     $&$-1.53_{-0.01}^{+0.01}  $&$   0.18 $&$ 0.068  $& Band   \\
\hline
\end{tabular}
 \end{center}
 $\rm F_{Ep.,1}$, $\rm F_{Ep.,2}$, $\rm F_{Ep.,1}$ and $\rm F_{Ep.,2}$ : in units of $\rm 10^{-6}$ $\rm erg~cm^{-2}~s^{-1}$;
 $\rm E_{iso, 1}$ and   $\rm E_{iso,2}$  : in units of $\rm 10^{52}$ $\rm erg$; $\rm L_{iso,1}$ and $\rm L_{iso,2}$ in units of $\rm 10^{52}$ $\rm erg$  $\rm s^{-1}$
\end{scriptsize}
\label{tab:two_episode_grbfits}
\end{table*}


==> GRB 190829A arxiv22May/table_xrt.tex <==
%\clearpage




\begin{table*}
\label{tab:xrt_bat}
\caption{Joint XRT and BAT, UVOT and XRT, XRT spectral best fit parameters}
%\setlength{\tabcolsep}{2pt}
\begin{tiny}
\begin{center}
%\centering
%\tiny
\begin{tabular}{c|c|c|c|cccc|cc}
\hline
\multicolumn{1}{c|}{Phase} &
\multicolumn{1}{c|}{Time} & \multicolumn{1}{c|}{Detectors} & \multicolumn{1}{c|}{Models} & \multicolumn{4}{c|}{Parameters} & \multicolumn{2}{c}{Statistics} \\
\hline
& $\rm (s)$ &  &  \sw{Tbabs*zTBabs*cflux}* &    $\rm N_{H} (z)$  & $\rm \Gamma$ ($\rm \Gamma_{1}$, $\rm \Gamma_{2}$) & $\rm E_c (E_{b})$ & $\rm kT_{BB} $&                     $\rm \chi^{2}$/dof & \sw{C-stat}/dof \\
\hline
 I & 104-228  & XRT (WT) & PL &      $0.76^{+0.22}_{-0.17}$ & $2.12_{-0.18}^{+0.20}$ & -- & --&-- &390.3/383 \\
 
 &  & & CPL      & $0.12_{-0.12}^{+0.20}$  & $-0.63_{-0.73}^{+0.81}$ & $1.12_{-0.27}^{+0.50}$ & --& --& 357.4/382   \\
  &  & BB + PL &    $0.04_{-0.04}^{+0.09}$  &$0.71_{-0.31}^{+0.52}$ & -- & $0.69^{+0.05}_{-0.05}$& --&354.5/382\\ 
  
%  & & BB+CPL &  $0.03^{+0.10}_{-0.03}$ & $-0.01^{+1.14}_{-1.08}$ & $5.02^{+\infty}_{-5.75}$ & $0.68^{+0.06}_{-0.07}$ &&--&354.5/381  \\   \hline

  && BAT + XRT (WT) & PL &  $0.84_{-0.20}^{+0.27}$ & $2.11_{-0.17}^{+0.20}$ & --& --&  125.1/103 &--    \\
&  &  & CPL &      $0.15^{+0.24}_{-0.16}$   & $-0.49^{+0.86}_{-0.81}$ & $1.21_{-0.32}^{+0.65}$ & --&  103.7/102 &--  \\
& & & BB + PL &      $0.06_{-0.06}^{+0.11}$  &$0.50_{-0.29}^{+0.64}$ & -- & $0.69_{-0.05}^{+0.06}$& 97.7/102 &--\\ 
%  & & BB+CPL& $0.05^{+0.12}_{-0.05}$ & $-0.06^{+0.99}_{-0.72}$  & $6.06^{+\infty}_{-5.49}$  &$0.68^{+0.07}_{-0.06}$&& 97.3/101  &\\ \hline \hline
 %&  & CPL      &  $1.19_{-0.12}^{0.13}$ & $1.47_{-0.26}^{+0.26}$ & $6.57_{-2.10}^{+5.67}$ &-- &&--& 811.1/757               \\

%& & BB + PL       & $0.90_{-0.14}^{+0.24}$ &$1.49_{-0.22}^{+0.31}$ & --& $0.61_{-0.04}^{+0.06}$&&--&798.8/756               \\
%&  & BB + CPL & $0.55_{-0.12}^{+0.08}$  & $-1.83_{-0.46}^{+1.34}$ &  $1.68_{-0.11}^{+0.13}$ & $0.57_{-0.10}^{+0.34}$&& -- &790.7/755               \\\hline\hline
%104-1700     & XRT (WT)          & PL     &  $1.35_{-0.07}^{+0.07}$ & $2.03_{-0.05}^{+0.05}$& -- &--                           &&--& 830.5/761               \\
 %&  & CPL & $1.06_{-0.11}^{+0.12}$ & $1.30_{-0.25}^{+0.25}$& $04.96_{-1.27}^{+2.54}$&-- && --& 806.3/760               \\
 %& & BB+PL       & $0.80_{-0.17}^{+0.17}$ &  $1.46_{-0.30}^{+0.24}$&--& $0.63_{-0.03}^{+0.04}$    && --&785.4/759               \\
 %&  & BB+CPL & $0.40_{-0.12}^{+0.13}$ &  $-2.11_{-0.35}^{+1.12}$& $1.69_{-0.13}^{+0.16}$ &  $0.55_{-0.06}^{+0.25}$ &&    --                       & 776.1/758           
% \hline\hline
%&   & CPL      &  $1.36_{-0.19}^{+0.20}$ &  $1.84_{-0.53}^{+0.30}$ & $13.84_{-9.33}^{-13.95}$&--&& --& 498.9/541               \\ 
%&  & BB+PL       & $1.23_{-0.31}^{+0.17}$ & $1.85_{-0.48}^{+0.44}$ &-- & $0.54_{-0.53}^{+1.06}$ &&-- & 497.7/540               \\  &   & BB+CPL & $0.85_{-0.24}^{+0.28}$ &  $-1.06_{-1.29}^{+2.45}$& $1.67_{-0.25}^{+0.44}$ & $0.65_{-0.23}^{+0.89}$  & & -- & 496.1/539               \\ 
%\hline
%.37 $\times 10^{4}$ - 1.67 $\times 10^{5}$ (IV a) & XRT (PC)   & PL &  $1.03_{-0.12}^{+0.13}$ &  $2.02_{-0.11}^{+0.12}$ & -- & --& --& 532.1/541               \\
%&   & CPL      &  $0.98_{-0.11}^{+0.05}$ &  $1.94_{-0.23}^{+0.13}$ & $66.07_{-99.08}^{+\infty}$&--&& --& 532.8/540              \\ 
%&  & \sw{bknpow}       & $1.03_{-0.12}^{+0.13}$ & $2.02_{-0.11}^{+0.12}$  & $18.54_{-18.54}^{+\infty}$ & -- &&-- & 532.1/539               \\  &  &        &  & $2.61_{-2.61}^{+\infty}$  &  &  && &                \\  \hline
%\hline
%1.67 $\times 10^{5}$ - 1.55 $\times 10^{6}$ (IV b) & XRT (PC)   & PL &  $1.12_{-0.12}^{+0.13}$ &  $2.35_{-0.13}^{+0.13}$ & -- & --& --& 486.76/489               \\
%&   & CPL      &  $1.18_{-0.12}^{+0.13}$ &  $2.34_{-0.14}^{+0.13}$ & $500_{-\infty}^{+\infty}$&--&& --& 486.8/488               \\ 
&  && \sw{bknpow}       & $1.27_{-0.15}^{+0.16}$ & $2.59_{-0.16}^{+0.18}$  & $4.93_{-0.72}^{+0.60}$ & -- &-- & 465.9/487               \\  &  &        &  & $0.40_{-1.04}^{+0.87}$  &  &  & &                \\ \hline
%896-10900  & XRT (WT $\&$ PC)   & PL &  $1.47_{-0.16}^{+0.17}$ &  $2.10_{-0.12}^{+0.12}$& -- & --&& --&499.6/542               \\
%147 - 620  & XRT (WT $\&$ PC) & PL    & $1.59_{-0.27}^{+0.31}$ & $2.46_{-0.22}^{+0.23}$& -- &--&&-- & 494.3/548               \\%\hline
III (pre) & 147 - 620  & XRT (WT $\&$ PC) & PL    & $1.59_{-0.27}^{+0.31}$ & $2.46_{-0.22}^{+0.23}$& -- &--&-- & 494.3/548               \\%\hline
&  && \sw{bknpow}       & $1.12_{-0.42}^{+0.21}$ & $1.77_{-0.73}^{+0.48}$  & $2.89_{-0.48}^{+0.62}$ & -- &-- & 486.0/546               \\  &  &        &  & $3.00_{-0.36}^{+0.60}$  &  &  &&                \\ 
III (rise) & 620 - 1140 & XRT (WT $\&$ PC) & PL    & $1.44_{-0.26}^{+0.29}$ & $2.18_{-0.21}^{+0.22}$& -- &--&-- & 583.8/554               \\%\hline
&  && \sw{bknpow}       & $1.45_{-0.18}^{+0.26}$ & $2.20_{-2.23}^{+\infty}$  & $0.48_{-0.08}^{+\infty}$ & -- &-- & 584/552              \\  &  &        &  & $2.20_{-0.21}^{+0.22}$  &  &  & &                \\               
III (top) & 1120-1700 & XRT (WT) & PL    & $1.42_{-0.08}^{+0.08}$ & $2.03_{-0.06}^{+0.06}$& -- &--&-- & 823.9/758               \\
&  & & \sw{bknpow}       & $1.07_{-0.21}^{+0.20}$ & $1.68_{-0.44}^{+0.30}$  & $2.46_{-0.38}^{+1.01}$ & -- &-- & 550.2/601               \\  &  &        &  & $2.11_{-0.13}^{+0.19}$  &    && &                \\ \hline
 \hline
Phase & Time & Detection &  \sw{redden*phabs*zdust*} &    $\rm N_{H} (z)$ & $\rm \Gamma$ ($\rm \Gamma_{1}$, $\rm \Gamma_{2}$) & $\rm  E_{b}$ & $\rm E_{B-V} $&                      $\rm \chi^{2}$/dof & \sw{C-stat}/dof \\
  & $\rm (s)$ &zphabs*   &    &  &                     &  \\
\hline
 III (pre) & 147 - 620  & (UVOT $\&$ XRT WT) & PL    & $0.86_{-0.20}^{+0.23}$ & $1.84_{-0.15}^{+0.14}$& -- &$1.14_{-0.28}^{+0.25}$&39.7/26 & --               \\
&  & &\sw{bknpow}       & $0.80_{-0.38}^{+0.32}$ & $1.50_{-0.54}^{+0.29}$  & $3.14_{-0.44}^{+0.85}$ & $0.67_{-0.63}^{+0.43}$ &  25.9/24& --              \\
 &  &        &  & $3.54_{-0.89}^{+3.54}$  &  &  & &                \\ %\hline
III (rise) & 620 - 1140 & (UVOT $\&$ XRT PC) & PL    & $1.26_{-0.23}^{+0.33}$ & $1.92_{-0.12}^{+0.21}$& -- &$1.08_{-0.25}^{+0.48}$&56.5/30 & --               \\
&  & &\sw{bknpow}       & 1.28 & 1.94  & 18.73 &1.11 & 56.4/28& --               \\ 
 &  &        &  & 2.30  &  &  & &                \\ %\hline
III (top) & 1120-1700 & (UVOT $\&$ XRT WT) & PL    & $1.41_{-0.07}^{+0.07}$ & $1.99_{-0.04}^{+0.05}$& -- &$1.33_{-0.10}^{+0.11}$&404.3/353 & --               \\
&  & &\sw{bknpow}       & $1.36_{-0.07}^{+0.07}$ & $1.84_{-0.06}^{+0.07}$  & $2.59_{-0.55}^{+0.81}$ & $1.04_{-0.12}^{+0.14}$ &378.9/351 & --              \\ 
 &  &        &  & $2.15_{-0.09}^{+0.17}$  &  &  & &                \\ 
III (decay) & 4860-23700 & (UVOT $\&$ XRT PC) & PL    & $0.96_{-0.06}^{+0.06}$ & $1.69_{-0.02}^{+0.03}$& -- &$0.56_{-0.04}^{+0.05}$&171.2/147 & --   \\
&  & &\sw{bknpow}       & $1.11_{-0.08}^{+0.10}$ & $1.64_{-0.03}^{+0.03}$  & $2.26_{-0.46}^{+0.63}$ & $0.52_{-0.04}^{+0.04}$ & 125.2/145& --           \\ 
 &  &        &  & $2.10_{-0.12}^{+0.19}$  &  &  & &                \\ 
\hline
IV (pre-break) & 2.37 $\times 10^{4}$ - 1.67 $\times 10^{5}$ & XRT (PC)   & PL &  $1.03_{-0.12}^{+0.13}$ &  $2.02_{-0.11}^{+0.12}$ & -- & --& --& 532.1/541               \\
IV (post-break) & 1.67 $\times 10^{5}$ - 1.55 $\times 10^{6}$ & XRT (PC)   & PL &  $1.12_{-0.12}^{+0.13}$ &  $2.35_{-0.13}^{+0.13}$ & -- & --& --& 486.76/489               \\

\hline

\end{tabular}
 \end{center}
All errors are quoted at 90\% confindence level.
 $\rm N_{H} (z)$ : in units of $\rm 10^{22}$ $\rm cm^{-2}$;
$\rm  E_{b}$, $\rm  E_{c}$ and $\rm kT_{BB} $ : in units of  $\rm keV$, where $\rm  E_{b}$ and $\rm  E_{c}$ are the break and cutoff energies, respectively. Reddening parameter in host is obtained for SMC extinction law. 
\end{tiny}
\end{table*}

==> table_lag.tex <==
\begin{table*}
\begin{center}
\caption{ Time lag w.r.t 150-300 keV photons label{lag_table}}
\begin{tabular}{c|c|c}
\hline
- & Episode-1 & Episode-2 \\
\hline
Energy Band & Lag(Correlation) & Lag(Correlation) \\
(keV) & (sec(\%)) & (sec(\%)) \\
\hline
\multicolumn{5}{c}{4ms timebin} \\
\hline
8-30 & $1.135\pm0.006(6.38\pm0.01)$ & $0.462\pm0.006(11.67\pm0.00)$ \\
30-50 & $0.848\pm0.006(4.84\pm0.01)$ & $0.618\pm0.021(8.49\pm0.00)$ \\
50-100 & $0.086\pm0.008(3.81\pm0.01)$ & $-0.047\pm0.003(4.59\pm0.01)$ \\
8-100 & $0.723\pm0.016(8.21\pm0.04)$ & $0.619\pm0.025(11.82\pm0.00)$ \\
\hline
\multicolumn{5}{c}{8ms timebin} \\
\hline
8-30 & $0.071\pm0.003(63.01\pm0.01)$ & $0.100\pm0.004(64.97\pm0.01)$ \\
30-50 & $-0.003\pm0.003(58.51\pm0.02)$ & $-0.042\pm0.005(60.96\pm0.01)$ \\
50-100 & $0.051\pm0.003(56.91\pm0.02)$ & $-0.083\pm0.002(56.89\pm0.02)$ \\
8-100 & $0.081\pm0.002(66.17\pm0.01)$ & $0.040\pm0.003(65.94\pm0.01)$ \\
\hline
\multicolumn{5}{c}{16ms timebin} \\
\hline
8-30 & $1.215\pm0.007(11.43\pm0.01)$ & $0.528\pm0.097(16.72\pm0.02)$ \\
30-50 & $0.717\pm0.008(8.98\pm0.01)$ & $0.454\pm0.038(13.82\pm0.01)$ \\
50-100 & $0.156\pm0.008(7.32\pm0.02)$ & $-0.048\pm0.004(8.40\pm0.01)$ \\
8-100 & $0.755\pm0.007(14.09\pm0.10)$ & $0.533\pm0.109(16.84\pm0.01)$ \\
\hline
\end{tabular}
\end{center}
\end{table*}


==> table_xrt.tex <==
%\clearpage




\begin{table*}
\label{tab:xrt_bat}
\caption{Joint XRT and BAT, UVOT and XRT, XRT spectral best fit parameters}
%\setlength{\tabcolsep}{2pt}
\begin{tiny}
\begin{center}
%\centering
%\tiny
\begin{tabular}{c|c|c|c|cccc|cc}
\hline
\multicolumn{1}{c|}{Phase} &
\multicolumn{1}{c|}{Time} & \multicolumn{1}{c|}{Detectors} & \multicolumn{1}{c|}{Models} & \multicolumn{4}{c|}{Parameters} & \multicolumn{2}{c}{Statistics} \\
\hline
& $\rm (s)$ &  &  \sw{Tbabs*zTBabs*cflux}* &    $\rm N_{H} (z)$  & $\rm \Gamma$ ($\rm \Gamma_{1}$, $\rm \Gamma_{2}$) & $\rm E_c (E_{b})$ & $\rm kT_{BB} $&                     $\rm \chi^{2}$/dof & \sw{C-stat}/dof \\
\hline
 I & 104-228  & XRT (WT) & PL &      $0.76^{+0.22}_{-0.17}$ & $2.12_{-0.18}^{+0.20}$ & -- & --&-- &390.3/383 \\
 
 &  & & CPL      & $0.12_{-0.12}^{+0.20}$  & $-0.63_{-0.73}^{+0.81}$ & $1.12_{-0.27}^{+0.50}$ & --& --& 357.4/382   \\
  &  & BB + PL &    $0.04_{-0.04}^{+0.09}$  &$0.71_{-0.31}^{+0.52}$ & -- & $0.69^{+0.05}_{-0.05}$& --&354.5/382\\ 
  
%  & & BB+CPL &  $0.03^{+0.10}_{-0.03}$ & $-0.01^{+1.14}_{-1.08}$ & $5.02^{+\infty}_{-5.75}$ & $0.68^{+0.06}_{-0.07}$ &&--&354.5/381  \\   \hline

  && BAT + XRT (WT) & PL &  $0.84_{-0.20}^{+0.27}$ & $2.11_{-0.17}^{+0.20}$ & --& --&  125.1/103 &--    \\
&  &  & CPL &      $0.15^{+0.24}_{-0.16}$   & $-0.49^{+0.86}_{-0.81}$ & $1.21_{-0.32}^{+0.65}$ & --&  103.7/102 &--  \\
& & & BB + PL &      $0.06_{-0.06}^{+0.11}$  &$0.50_{-0.29}^{+0.64}$ & -- & $0.69_{-0.05}^{+0.06}$& 97.7/102 &--\\ 
%  & & BB+CPL& $0.05^{+0.12}_{-0.05}$ & $-0.06^{+0.99}_{-0.72}$  & $6.06^{+\infty}_{-5.49}$  &$0.68^{+0.07}_{-0.06}$&& 97.3/101  &\\ \hline \hline
 %&  & CPL      &  $1.19_{-0.12}^{0.13}$ & $1.47_{-0.26}^{+0.26}$ & $6.57_{-2.10}^{+5.67}$ &-- &&--& 811.1/757               \\

%& & BB + PL       & $0.90_{-0.14}^{+0.24}$ &$1.49_{-0.22}^{+0.31}$ & --& $0.61_{-0.04}^{+0.06}$&&--&798.8/756               \\
%&  & BB + CPL & $0.55_{-0.12}^{+0.08}$  & $-1.83_{-0.46}^{+1.34}$ &  $1.68_{-0.11}^{+0.13}$ & $0.57_{-0.10}^{+0.34}$&& -- &790.7/755               \\\hline\hline
%104-1700     & XRT (WT)          & PL     &  $1.35_{-0.07}^{+0.07}$ & $2.03_{-0.05}^{+0.05}$& -- &--                           &&--& 830.5/761               \\
 %&  & CPL & $1.06_{-0.11}^{+0.12}$ & $1.30_{-0.25}^{+0.25}$& $04.96_{-1.27}^{+2.54}$&-- && --& 806.3/760               \\
 %& & BB+PL       & $0.80_{-0.17}^{+0.17}$ &  $1.46_{-0.30}^{+0.24}$&--& $0.63_{-0.03}^{+0.04}$    && --&785.4/759               \\
 %&  & BB+CPL & $0.40_{-0.12}^{+0.13}$ &  $-2.11_{-0.35}^{+1.12}$& $1.69_{-0.13}^{+0.16}$ &  $0.55_{-0.06}^{+0.25}$ &&    --                       & 776.1/758           
% \hline\hline
%&   & CPL      &  $1.36_{-0.19}^{+0.20}$ &  $1.84_{-0.53}^{+0.30}$ & $13.84_{-9.33}^{-13.95}$&--&& --& 498.9/541               \\ 
%&  & BB+PL       & $1.23_{-0.31}^{+0.17}$ & $1.85_{-0.48}^{+0.44}$ &-- & $0.54_{-0.53}^{+1.06}$ &&-- & 497.7/540               \\  &   & BB+CPL & $0.85_{-0.24}^{+0.28}$ &  $-1.06_{-1.29}^{+2.45}$& $1.67_{-0.25}^{+0.44}$ & $0.65_{-0.23}^{+0.89}$  & & -- & 496.1/539               \\ 
%\hline
%.37 $\times 10^{4}$ - 1.67 $\times 10^{5}$ (IV a) & XRT (PC)   & PL &  $1.03_{-0.12}^{+0.13}$ &  $2.02_{-0.11}^{+0.12}$ & -- & --& --& 532.1/541               \\
%&   & CPL      &  $0.98_{-0.11}^{+0.05}$ &  $1.94_{-0.23}^{+0.13}$ & $66.07_{-99.08}^{+\infty}$&--&& --& 532.8/540              \\ 
%&  & \sw{bknpow}       & $1.03_{-0.12}^{+0.13}$ & $2.02_{-0.11}^{+0.12}$  & $18.54_{-18.54}^{+\infty}$ & -- &&-- & 532.1/539               \\  &  &        &  & $2.61_{-2.61}^{+\infty}$  &  &  && &                \\  \hline
%\hline
%1.67 $\times 10^{5}$ - 1.55 $\times 10^{6}$ (IV b) & XRT (PC)   & PL &  $1.12_{-0.12}^{+0.13}$ &  $2.35_{-0.13}^{+0.13}$ & -- & --& --& 486.76/489               \\
%&   & CPL      &  $1.18_{-0.12}^{+0.13}$ &  $2.34_{-0.14}^{+0.13}$ & $500_{-\infty}^{+\infty}$&--&& --& 486.8/488               \\ 
&  && \sw{bknpow}       & $1.27_{-0.15}^{+0.16}$ & $2.59_{-0.16}^{+0.18}$  & $4.93_{-0.72}^{+0.60}$ & -- &-- & 465.9/487               \\  &  &        &  & $0.40_{-1.04}^{+0.87}$  &  &  & &                \\ \hline
%896-10900  & XRT (WT $\&$ PC)   & PL &  $1.47_{-0.16}^{+0.17}$ &  $2.10_{-0.12}^{+0.12}$& -- & --&& --&499.6/542               \\
%147 - 620  & XRT (WT $\&$ PC) & PL    & $1.59_{-0.27}^{+0.31}$ & $2.46_{-0.22}^{+0.23}$& -- &--&&-- & 494.3/548               \\%\hline
III (pre) & 147 - 620  & XRT (WT $\&$ PC) & PL    & $1.59_{-0.27}^{+0.31}$ & $2.46_{-0.22}^{+0.23}$& -- &--&-- & 494.3/548               \\%\hline
&  && \sw{bknpow}       & $1.12_{-0.42}^{+0.21}$ & $1.77_{-0.73}^{+0.48}$  & $2.89_{-0.48}^{+0.62}$ & -- &-- & 486.0/546               \\  &  &        &  & $3.00_{-0.36}^{+0.60}$  &  &  &&                \\ 
III (rise) & 620 - 1140 & XRT (WT $\&$ PC) & PL    & $1.44_{-0.26}^{+0.29}$ & $2.18_{-0.21}^{+0.22}$& -- &--&-- & 583.8/554               \\%\hline
&  && \sw{bknpow}       & $1.45_{-0.18}^{+0.26}$ & $2.20_{-2.23}^{+\infty}$  & $0.48_{-0.08}^{+\infty}$ & -- &-- & 584/552              \\  &  &        &  & $2.20_{-0.21}^{+0.22}$  &  &  & &                \\               
III (top) & 1120-1700 & XRT (WT) & PL    & $1.42_{-0.08}^{+0.08}$ & $2.03_{-0.06}^{+0.06}$& -- &--&-- & 823.9/758               \\
&  & & \sw{bknpow}       & $1.07_{-0.21}^{+0.20}$ & $1.68_{-0.44}^{+0.30}$  & $2.46_{-0.38}^{+1.01}$ & -- &-- & 550.2/601               \\  &  &        &  & $2.11_{-0.13}^{+0.19}$  &    && &                \\ \hline
 \hline
Phase & Time & Detection &  \sw{redden*phabs*zdust*} &    $\rm N_{H} (z)$ & $\rm \Gamma$ ($\rm \Gamma_{1}$, $\rm \Gamma_{2}$) & $\rm  E_{b}$ & $\rm E_{B-V} $&                      $\rm \chi^{2}$/dof & \sw{C-stat}/dof \\
  & $\rm (s)$ &zphabs*   &    &  &                     &  \\
\hline
 III (pre) & 147 - 620  & (UVOT $\&$ XRT WT) & PL    & $0.86_{-0.20}^{+0.23}$ & $1.84_{-0.15}^{+0.14}$& -- &$1.14_{-0.28}^{+0.25}$&39.7/26 & --               \\
&  & &\sw{bknpow}       & $0.80_{-0.38}^{+0.32}$ & $1.50_{-0.54}^{+0.29}$  & $3.14_{-0.44}^{+0.85}$ & $0.67_{-0.63}^{+0.43}$ &  25.9/24& --              \\
 &  &        &  & $3.54_{-0.89}^{+3.54}$  &  &  & &                \\ %\hline
III (rise) & 620 - 1140 & (UVOT $\&$ XRT PC) & PL    & $1.26_{-0.23}^{+0.33}$ & $1.92_{-0.12}^{+0.21}$& -- &$1.08_{-0.25}^{+0.48}$&56.5/30 & --               \\
&  & &\sw{bknpow}       & 1.28 & 1.94  & 18.73 &1.11 & 56.4/28& --               \\ 
 &  &        &  & 2.30  &  &  & &                \\ %\hline
III (top) & 1120-1700 & (UVOT $\&$ XRT WT) & PL    & $1.41_{-0.07}^{+0.07}$ & $1.99_{-0.04}^{+0.05}$& -- &$1.33_{-0.10}^{+0.11}$&404.3/353 & --               \\
&  & &\sw{bknpow}       & $1.36_{-0.07}^{+0.07}$ & $1.84_{-0.06}^{+0.07}$  & $2.59_{-0.55}^{+0.81}$ & $1.04_{-0.12}^{+0.14}$ &378.9/351 & --              \\ 
 &  &        &  & $2.15_{-0.09}^{+0.17}$  &  &  & &                \\ 
III (decay) & 4860-23700 & (UVOT $\&$ XRT PC) & PL    & $0.96_{-0.06}^{+0.06}$ & $1.69_{-0.02}^{+0.03}$& -- &$0.56_{-0.04}^{+0.05}$&171.2/147 & --   \\
&  & &\sw{bknpow}       & $1.11_{-0.08}^{+0.10}$ & $1.64_{-0.03}^{+0.03}$  & $2.26_{-0.46}^{+0.63}$ & $0.52_{-0.04}^{+0.04}$ & 125.2/145& --           \\ 
 &  &        &  & $2.10_{-0.12}^{+0.19}$  &  &  & &                \\ 
\hline
IV (pre-break) & 2.37 $\times 10^{4}$ - 1.67 $\times 10^{5}$ & XRT (PC)   & PL &  $1.03_{-0.12}^{+0.13}$ &  $2.02_{-0.11}^{+0.12}$ & -- & --& --& 532.1/541               \\
IV (post-break) & 1.67 $\times 10^{5}$ - 1.55 $\times 10^{6}$ & XRT (PC)   & PL &  $1.12_{-0.12}^{+0.13}$ &  $2.35_{-0.13}^{+0.13}$ & -- & --& --& 486.76/489               \\

\hline

\end{tabular}
 \end{center}
All errors are quoted at 90\% confindence level.
 $\rm N_{H} (z)$ : in units of $\rm 10^{22}$ $\rm cm^{-2}$;
$\rm  E_{b}$, $\rm  E_{c}$ and $\rm kT_{BB} $ : in units of  $\rm keV$, where $\rm  E_{b}$ and $\rm  E_{c}$ are the break and cutoff energies, respectively. Reddening parameter in host is obtained for SMC extinction law. 
\end{tiny}
\end{table*}
